Spectral study of V565 Mon: Probable FU Ori-like or chemically peculiar star

We present the detailed spectroscopic study of V565 Mon pre-main-sequence star, which is the illuminating star of Parsamian 17 cometary nebula. Observations were performed with 2.6 m telescope in Byurakan Astrophysical Observatory in 15 February 2018. Radial velocities and equivalent widths of the most prominent lines of V565 Mon are presented. We built the spectral energy distribution and estimated the main parameters of the star, for example obtained bolometric luminosity of V565 Mon is $L_{V565}\approx 130L_{\odot} $ . Considering all features of V565 Mon we came to conclusion that this young intermediate-mass star can belongs to some intermediate class between T Tau and HAeBe stars. Very unusual for a young star is the presence of strong absorption Ba II lines in the spectrum. Possible explanations on this issue are discussed. Hence, we think that V565 Mon is a unique example, which can help to understand some open questions in nucleosynthesis problem in young stars.

==> readme <==
Dear Colleagues: 

The final publication layout will be produced by using raa.cls. 
Therefore, we strongly encourage you to prepare your LaTeX manuscript 
with this class file. Please unpack raa-package.tar.gz, it includes 

raa.cls        ---- RAA macro class file for LaTeX2e 
sample.tex     ---- a sample file using raa.cls (LaTeX source) 
sample.ps      ---- the PS file created by sample.tex in referee format  
sample.pdf     ---- the PDF file created by sample.tex in referee format  
readme         ---- this file  
f?.eps         ---- three demo figures used in the LaTeX template source
sample2.tex    ---- a sample file for using raa.bst
sample2_fig?.eps -- two demo figures used in sample2.tex
sample2.pdf    ---- the PDF file created by sample.tex in referee format
sample2.bbl    ---- bibliography file using by sample2.tex
bibtex.bib     ---- an example for bibtex file

natbib.sty     ---- This package reimplements the LaTeX \cite command
natnotes.pdf   ---- Brief reference sheet for Natbib (pdf)
raa.bst        ---- Bibliography style file 

Hope you enjoy the use of this macro. Your suggestions and comments are 
highly welcome. Thanks.

Editorial Office
E-mail:  raa@raa-journal.org

